ELUDE: Generating interpretable explanations via a decomposition into labelled and unlabelled features

Deep learning models have achieved remarkable success in different areas of machine learning over the past decade; however, the size and complexity of these models make them difficult to understand. In an effort to make them more interpretable, several recent works focus on explaining parts of a deep neural network through human-interpretable, semantic attributes. However, it may be impossible to completely explain complex models using only semantic attributes. In this work, we propose to augment these attributes with a small set of uninterpretable features. Specifically, we develop a novel explanation framework ELUDE (Explanation via Labelled and Unlabelled DEcomposition) that decomposes a model's prediction into two parts: one that is explainable through a linear combination of the semantic attributes, and another that is dependent on the set of uninterpretable features. By identifying the latter, we are able to analyze the "unexplained" portion of the model, obtaining insights into the information used by the model. We show that the set of unlabelled features can generalize to multiple models trained with the same feature space and compare our work to two popular attribute-oriented methods, Interpretable Basis Decomposition and Concept Bottleneck, and discuss the additional insights ELUDE provides.

==> CAM_cub.tex <==




==> figures/splash.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\textwidth]{CompleteInterpretability-2/figs/pull_global_local.png}
\caption{Given an image classification model and a set of labelled attributes (like \texttt{fur} or \texttt{paw}), our proposed method ELUDE decomposes the prediction of a class like \texttt{cat} into information gained from labelled attributes and information gained from visual features other than these attributes. This allows us to generate both a global explanation of general attributes important to a class (\emph{left}) as well as a local explanation of how each attribute and learned feature contributes to the overall prediction (\emph{right}).} %\olga{I like the figure a lot. A couple of thoughts: (1) it's a little verbose, particularly the ``can't'' part. See if we can cut out some words there, e.g., just remove the ``about the prediction''. Also, standardize ``available'' vs ''given'' and ``labeled'' vs ``annotated'' (also vs ''semantic'') attributes. (2) I wonder if it's possible to make it just a tiny bit more complicated, e.g., show two GradCAMs corresponding to a rank-2 U. Since this doubles as a methods figure,  it would be good to not quite have it be so simple. (3) Can take up less vertical space (the gray box should be two rows rather than 4, which would allow everything else to come up higher, or make space for a more complicated explanation) } 
\label{fig:pull_fig}
\end{figure}
%\footnotetext{The image of the cat in the figure was taken from \url{https://www.pexels.com/photo/a-cute-cat-lying-on-a-cushion-inside-the-carton-box-7607355/}}

==> sections/experiments_prev.tex <==
Given access to labelled semantic attributes and a trained model, we want to describe what can and \emph{cannot} be explained about the model using these attributes. In this section, we demonstrate the effectiveness of our method on two different settings. We first describe the datasets and models on which we test our method, and then provide results for each setting.

\smallsec{Models and attributes}We test our method of interpretability on two different settings. The first setting we test is an interpretable-by-design model developed by Koh \etal~\cite{koh2020conceptbottleneck}. This model is trained on the CUB dataset~\cite{WahCUB_200_2011} that comprises of 200 different types of birds, labelled with 312 semantic attributes. Koh \etal create a model that first predicts the semantic attributes, and then use these attribute predictions to predict the class of the image. They test different methods of training such a model: training the attribute predictor first and then the class predictor with the ground truth labels, training them separately, but using the outputs of the attribute predictor as inputs to the class predictor, and  training both jointly. In our experiments, we use the trained weights provided by the author for the joint model with the concept loss weight = 1. This model is very similar to our explanation, wherein we predict a model's behaviour by approximating it with a linear combination of the semantic attributes. However, rather than changing any of the model weights, we only provide an post-hoc global explanation of the model. We choose this model to understand what more our method can convey beyond the model's dependence on the semantic attributes. 

The second model we explain is a ResNet18~\cite{he2016resnet} network trained on Places365 using the ADE20k dataset~\cite{zhou2017ade20k,zhou2019ade20k_ijcv}, which is labelled with attributes from various categories like color, texture, objects and object parts. This is arguably a more complex model, working with images that contain multiple objects. We examine which of these objects impact the model's scene classification. 

\smallsec{Implementation details}
For the ADE20k dataset~\cite{zhou2017ade20k}, we split the dataset randomly into train (60\%), val (20\%), and test (20\%) splits to use for the classifiers. For the CUB dataset~\cite{WahCUB_200_2011}, we use just the test set (splitting it randomly into train (60\%), val (20\%) and test (20\%)) for our analysis, since the model is trained on the training set of this dataset, and the distribution of the scores (as well as the accuracy) on the training set and test set are very different in general.  For both datasets,  we use the validation set to test different values of $\epsilon$, the error threshold we use for the semantic attribute classifiers we learn from $f(X)$. 

For the concept bottleneck model, we use the features output by the attribute layer as $f(X)$, and the 312 labelled attributes as $A$. For the Places365 model, we use the features output after the average pool layer in the resnet18 model as $f(X)$, and the concepts labelled in the Broden dataset~\cite{bau2017netdissect} as $A$. 
 
For all the linear classifiers learned, we use scikit-learn's~\cite{scikit-learn} Logistic Regression model, with the default parameters.
%\olga{do we tune the regularization threshold?} \vikram{No}
We train the attribute predictors with $f(X)$ as input and the ground truth labels for the attributes as output. We train $h$ to approximate the classification decision of model we provide an explanation for, i.e, $F(X)$. 
%\olga{how precisely is $h$ learned? E.g., is it approximating the classification score, or the classification decision?}

\subsection{CUB dataset}
%\vikram{does analysing conceptbottleneck here make sense? Are we saying something like the features encodes more information than what is present for the concepts which lets it work?}
In this section, we analyze an interpretable-by-design model developed by Koh \etal~\cite{koh2020conceptbottleneck}. This model focuses on predicting the semantic attributes, and then using these attributes to make a final prediction, similar to our explanation.  We find that while this model goes a long way into identifying important attributes used by the model, our method allows us to filter out some attributes that are not identifiable beyond random chance. Moreover, as the authors note in their paper, the continuous nature of the attribute predictions proves to be crucial to their model's success (flattening the predictions by adding a sigmoid layer to the attribute predictions does significantly worse). Our method identifies features within these  continuous predictions that are used by the model to make a prediction.  

\smallsec{Completeness of the explanation}

We find that 103 attributes can be learned from the feature space (more than random chance, i.e, above $0.5\%$ over random chance). We find that these attributes can only approximate the model's prediction $32.8\%$ of the time, suggesting that these features are not sufficient to predict the model's output. 
Moreover, the feature space contains 3 other dimensions that are not correlated with any of the attributes. Adding these features to the linear model allows us to predict the model output with an accuracy of 61.9\%. 

\begin{table}[t]
\centering
\input{cub_imp}
\caption{This table shows the number of times an attribute is among the top 10 most important attributes for each species of bird, for the  top set of attributes. We see that the three remaining CNN features still feature predominantly. Moreover, the feature \texttt{shape::perching-like} (which does not appear to be a causal attribute) is also deemed important}
\label{tab:cub_imp}
\end{table}


Table~\ref{tab:cub_imp} shows the number of times an attribute is among the top 10 most important attributes for each species of bird, for the top set of attributes. We see that the CNN features (which can't be used to predict any of the attributes) are still the most important features. Also concerning is the importance of \texttt{shape::perching-like}, which appears to be the way certain birds are pictured. The other important features seem to be the colors of different part of the bird, and the shape of the beak. 

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.5\textwidth]{CompleteInterpretability/figs/features_accuracy_tradeoff.png}
     \caption{Our method assumes that the attribute cannot be learned when the accuracy drops below a certain threshold, which we set as $\epsilon$ more than a random chance model. We plot the accuracy of a linear model trained on different types of features learned using our method to predict the baseline model's output at different values of $\epsilon$. We find that if we allow $\epsilon$ to be larger than $0.7\%$, the accuracy of our final explanation is very close to that of not using any of the semantic attributes, suggesting that this model does not depend on the semantic attributes much. }
     \label{fig:trade-off}
 \end{figure}


\smallsec{Low accuracy of our explanation} We investigate the low accuracy of our explanation. Our method has a hyperparameter -- when learning the linear classifiers, we assume that the attribute cannot be learned when the accuracy drops below a certain threshold. Decreasing this threshold gives us explanations that depend more on the semantic attributes. We set this threshold as  $\epsilon$ more than a random chance model. We demonstrate the trade-off between depending on the CNN features and semantic attributes in figure~\ref{fig:trade-off}, when varying $\epsilon$. We plot the accuracy of a linear model trained to predict the baseline model's output using (1) all the features in the baseline CNN, (i.e, the best that any linear explanation can do) (2) the features from the learned subspace that contain no information about the semantic attributes, and (3) the features from the learned subspace and the attributes that are learn-able from the feature space (i.e, our final explanation). We notice that once we allow $\epsilon$ to be larger than $0.7\%$, the linear models trained on the learned subspace and the linear model trained on the learned subspace and the learn-able attributes perform almost at the same accuracy, suggesting that the attributes do not contribute much to the explanation. Hence, when analyzing attribute importance, we use a slightly lower value of $\epsilon$, as 0.5\%; i.e, we assume that the feature space does not contain any information about an attribute when it has an accuracy of less than 0.5\% more than a random chance model.  


\begin{figure*}[t]
\centering
\input{pca_cub}
\caption{The three maximally and minimally activated images for each direction identified by PCA on the remaining uninterpretable features. The background appears to be the common feature for each, for example, the second set of images on row 1 are birds surrounded by green leaves, the second set of images in row 3 are birds perched on a stick, in a clear background.}
\label{fig:pca_cub}
\end{figure*}

\smallsec{Exploring the uninterpretable features}
\iffalse
We first probe the new 3 dimensional subspace using GradCAM~\cite{selvaraju2017gradcam}. Unlike the Places365 model visualization, we find that for CUB, the heatmap focus does not change that much from the original image (see ~\ref{fig:cam_cub} for a sample of 8 image pairs). Moreover, the average cosine similarity between the pairs is 0.87, much higher than the numbers seen on ADE20k. This might be because of the nature of this dataset -- CUB has a single object per image, unlike ADE20k. 

\begin{figure}[t]
    \centering
    \input{CompleteInterpretability/CAM_cub}
    \caption{We visualize GradCAM~\cite{selvaraju2017gradcam} heatmaps for the original model as well our explanation. In this case, we find that the heatmaps do not change much. }
    \label{fig:cam_cub}
\end{figure}
\fi 


In order to explore the remaining features, we perform PCA on this feature space. Figure~\ref{fig:pca_cub} contains images that maximally and minimally activate each direction. The background appears to be the most salient feature for most of these, suggesting that the classifier still makes it's prediction based on spurious correlations. 


\smallsec{Contrasting the interpretable-by-design model with a baseline model} We also run our method on a baseline ResNet18 model trained on the same dataset, to understand how these models differ. We find that the concept bottleneck model does indeed recognize more attributes from the CUB dataset compared to a baseline model (103 vs 60), and these 60 attributes can only predict the baseline model's output 24.9\% of the time. Our final explanation matches the prediction \olga{unfinished sentence?} Moreover, adding the 60 semantic attributes to the features only increases the accuracy by less than 0.3\%, suggesting that the baseline model does not use these attributes to make its final prediction.  

\subsection{Scene classification using Broden~\cite{bau2017netdissect} attributes}
For our next set of experiments, we provide an explanation for ResNet18 model trained on Places365~\cite{zhou2017places}, using the semantic attributes labelled in the Broden~\cite{bau2017netdissect}. In order to learn linear maps, we use the ADE20k~\cite{zhou2017ade20k,zhou2019ade20k_ijcv} dataset. We find that out of the 584 different attributes only 47 of them can be learned better than random chance. We also find a 227 dimension subspace of the feature space that cannot learn these attributes at all, and hence, our final explanation is on a 274 (227+47) dimension space. 

\smallsec{Completeness of our explanation} We find that our explanation matches the model's prediction on $73.6\%$ of the images.\footnote{A linear model learned on $f(X)$ to predict $g(f(X))$ has an accuracy of $77.5\%$ for this dataset / model combination, suggesting that that is the best possible any explanation can do.}. A linear model trained on just the semantic attributes to predict the model's output has an accuracy of 52.2\%. 
\begin{table*}[t]
    \centering
    \input{CompleteInterpretability/tables/ade20k_imp}
    \caption{The three most important attributes for each scene group, based on the weight of the linear model learned, along with the true positive rate for each. \texttt{cnn-feature} denotes that a dimension from $\mathbb{R}^{D'}$ was very important4
    . Attributes with positive weights are in \textcolor{NavyBlue}{\textbf{\texttt{blue}}} , attributes with negative weights are in \textcolor{red}{\textit{\texttt{red}}}. For most part, we see that the attributes match our intuition of what we would expect -- \texttt{bed} is important for \texttt{home-hotel}, \texttt{grass} and \texttt{trees} are important for \texttt{forest-field-jungle}. We also notice that the set of labelled attributes covers certain scenes better than others; forcing the others to rely on the remaining CNN features.  }
    \label{tab:ade20ktpr}
\end{table*}
We also notice that certain scene groups are easier for us to explain than others (Table~\ref{tab:ade20ktpr}), for example the scenes grouped under \texttt{home-hotel} has a much higher true positive rate (92.1\%) compared to \texttt{industrial-construction}, which only has a true positive rate of 48.2\%. We also consider the attributes that have the highest weights in our explanation for each scene category, to understand how the model makes its prediction. We note that most of these are as expected: \texttt{home-hotel} depends on \texttt{bed}; \texttt{water-ice-snow} depends on not having \texttt{buildings}, but having \texttt{sea}. Moreover, we see that our set of semantic attributes better captures certain classes than others: none of the top three important features for the class \texttt{industrial-construction} are semantic attributes. 



\smallsec{Exploring the uninterpretable features}
Our explanation gives us a subspace of the feature space of a CNN, however, we still are unclear on what this subspace encodes. We probe this subspace in two ways in order to gain some more insights into other potential attributes that the model could be using. For the first, we apply GradCAM(\cite{selvaraju2017gradcam}) on the explanation to understand what regions of the image are highlighted. We find that this highlights very different regions than the model (see Figure \ref{fig:cam_ade}, where we show pairs of regions activated by GradCAM on the baseline model and on our explanation model), often highlighting regions in the edges of the image.   

\begin{figure*}[t]
    \centering
    \input{CompleteInterpretability/tables/CAM_ade}
    \caption{For each category, we visualize the GradCAM on the baseline model, as well as our explanation. The GradCAM on our explanation shows us how much the model depends on these regions on the image in addition to the semantic attributes labelled. In this figure, we display six out of the 16 categories. We find that there are certain categories and images for which the heatmaps appears almost the same (for example, pairs that are bounded by red boxes), but there are others where the heatmaps are very different (examples bounded by blue boxes)}
    \label{fig:cam_ade}
\end{figure*}

%In order to understand when the GradCAM focus on the image changes, we compare the cosine similarity between the original and new heatmaps for each scene category. We compare this similarity value to that the true positive rate for each category, when using a linear model on just the semantic attributes to approximate the baseline model. As expected, we find that there is a negative correlation between the two: categories that have a high true positive rate do not rely on regions of the image anymore, and the GradCAM maps are thus more dissimilar. Figure~\ref{fig:ade_cosinetpr} shows this correlation. 
\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{CompleteInterpretability/figs/ade_cam_cosine_vs_tpr.png}
    \caption{In this graph, we plot the cosine similarity between the heatmaps generated by GradCAM\cite{selvaraju2017gradcam} on the original baseline model and the explanation generated by our method. We find that the true positive rate of a linear explanation on the semantic attributes correlates with this cosine similarity}% (pearson coefficient = $-0.32$)}
    \label{fig:ade_cosinetpr}
\end{figure}
Interestingly, the categories \texttt{indoor-sports-leisure}, \texttt{mountains-desert-sky} and \texttt{shopping-dining} have a much larger drop in cosine similarity compared to other categories with similar TPRs. \todo{possible reason?} 
\end{comment}


The other method we use to visualize the subspace is by looking at images that maximally / minimally activate PCA directions of the projected features. This allows us to understand what attributes might be encoded within these features. For example Table~\ref{tab:pca_ade} shows five out of the 25 main directions, each of which appears to be activated by an attribute not included within $A$. 

\begin{table}[t]
    \centering
\include{pca_ade20k}
    \caption{When viewing the images that maximally and minimally activate each PCA direction, we find that certain directions appear to correspond to human identifiable semantic concepts. 6 of these are displayed here, along with the tentative labels. }
    \label{tab:pca_ade}
\end{table}


\smallsec{Comparison with NetDissect~\cite{bau2017netdissect}}
We contrast the explanation our method provides, with that of NetDissect~\cite{bau2017netdissect}. NetDissect identifies neurons that activate regions that correlate with different concepts. Using their provided code\footnote{\url{https://github.com/CSAILVision/NetDissect-Lite}}, we find neurons in a Places365 trained ResNet18 model that correspond to attributes in Broden. We find that out of the 512 neurons in the penultimate layer, 82 respond strongly (using their definition of an IOU of greater than 0.04) to a total of 27 concepts, explaining around 16\% of the network. Moreover, all of these correspond to a `texture` attribute. While NetDissect allows us to identify human-identifiable concepts embedded in the network, our method also lets us understand how these concepts influence the model's prediction. 




==> sections/introduction_old.tex <==
\begin{comment}
* Need for interpretability
* Set scene as to what's currently happening in interpretability space
\end{comment}

In the past decade, deep learning has transformed the field of machine learning with its strong predictive capabilities.
As a result of its many recent successes, deep neural networks are increasingly being applied to high-impact, high-risk domains ranging from precision medicine to autonomous driving.
However, the highly parameterized nature of deep learning that fuels its predictive power also makes these networks challenging to understand.
The ability to thoroughly understand these models is crucial for engendering trust in them as well as for debugging and fixing undesired model behavior.

\begin{comment}
Deep learning models achieve excellent performance across a wide range of tasks. 
However, the gain in performance is accompanied by a lack of transparency-- these models remain notoriously difficult to understand, and often are treated as black boxes. 
This makes them unsuitable to be used in the real-world, especially when making high-stakes decisions, such as those for healthcare or self-driving cars\cite{}. 
Despite high performance on existing benchmarks, interpretability remains a key roadblock in unlocking the full potential of deep learning. 
\end{comment}


A number of works have focused on interpreting deep neural networks by labelling parts of a network with human-interpretable concepts. 
These can be categorized into two broad approaches:
First, some methods~\cite{bau2017netdissect,fong2018net2vec} focus on labelling individual neurons and/or combinations of neurons with concepts post-hoc (i.e., after a network has been trained).
Second, other works propose replacing traditional networks with interpretable-by-design models that explicitly use labelled concepts~\cite{koh2020conceptbottleneck} or learned ones~\cite{chen2018protopnet,nauta2021prototree}. 
Labelled concepts typically range from low-level concepts like colors and texture (e.g., \texttt{red}, \texttt{spotted}) to high-level semantic concepts like parts of objects, objects, and scenes (e.g., \texttt{ear}, \texttt{dog}, \texttt{sky}), whereas learned concepts are typically defined by prototypical examples that are image patches from the training set.  In Tab.~\ref{tab:review}, we summarize these lines of work and compare them to our proposed work.
%\ruth{This last sentence might be too detailed but I thought it could be helpful to the reader to have an intuition about what a concept is.} \olga{looks excellent}

\input{figures/splash}
\begin{comment}
Many methods have been proposed to explain a network's decision (for example, see \cite{qin2018convolutional,nguyen2019understanding} for brief surveys). The methods range from visualizing pixels / superpixels that contribute to a decision~\cite{ribeiro2016lime,zeiler2014visualizing,simonyan2013saliency,zhou2016cam,selvaraju2017gradcam,chattopadhay2018gradcamplusplus}, identifying neurons / combinations of neurons that align with certain concepts~\cite{bau2017netdissect,fong2018net2vec} as well as designing models that are interpretable-by-design~\cite{chen2018protopnet,koh2020conceptbottleneck,nauta2021prototree}. They have also been evaluated in several ways, both qualitative and quantitative, including human studies~\cite{selvaraju2017gradcam,bau2017netdissect}, correlations with pre-annotated regions~\cite{}
The proliferation of interpretability methods is heartening, with each one bringing unique strengths, insights and evaluation metrics.
\end{comment}

\begin{comment}
* We want a global explanation of the model. 
    * Need to use but also constrained by semantic attributes. 
    * Also want to start explaining more complicated models (multi-class, multi-head, etc.)

\end{comment}

Both types of approaches focus on quantifying and discovering the parts of a model's decision that \emph{can} be explained.
However, very few works have characterized what \emph{cannot} be explained by these techniques.
Such analysis would inform how models can be improved in terms of interpretability, in a similar way to how works analyzing the \emph{errors} of object detection~\cite{hoiem2012error,bolya2020tide} led to model improvements.



\begin{comment}
Something in common among all these methods is the focus on quantifying and discovering what \emph{can} be explained about the model's decisions. Every method explores and summarizes the discovered patterns that are correlated with the network's predictions, and notes that the network is not yet fully explained. However, what is frequently missing is the analysis of what \emph{cannot} be explained by each method. On one hand, explaining more and more of the network is the key goal of interpretability so it makes sense to focus on the positive explanations. On the other, as we argue in this work, there is a lot of overlooked value in quantifying and analyzing what patterns cannot yet be explained by the semantic attributes. For example, we identify patterns within the feature space that are relevant to the model's prediction (such as `passage` or `slanted roof`) that are not part of the attribute set, but that the model uses in order to make it's prediction. 
This is similar in spirit to works analyzing the \emph{errors} of object detection~\cite{hoiem2012error,bolya2020tide}, where identifying the types of errors the model makes helps us better the model. 
\end{comment}

\begin{comment}
Contributions:
*  Develop a method for identifying which concepts are meaningful for prediction and by how much
* Develop a framework for learning the portion of representation space unexplained by a concept set
* Analyze unexplained subspace using visualization techniques
* Compare against other popular concept-oriented interpretability works (primarily NetDissect and Concept Bottleneck).
\end{comment}

In this paper, we develop a novel interpretability paradigm named 
ELUDE (Explanation via a Labelled and Unlabelled DEcomposition) and make three contributions:
First, we develop a framework for learning a subspace of the model's feature space that \emph{cannot} be explained by a given set of concepts.
Second, we analyze the ``unexplained'' parts of a model's decision using various visualization techniques and qualitatively characterize the ``unexplained''  information that is meaningfully used by the model.
Third, we analyze how well this subspace generalizes to other models that are trained on the same feature space. 


%\input{CompleteInterpretability/tables/tab-review}

ELUDE identifies the parts of a network's prediction that can and cannot be explained by a set of pre-labelled semantic concepts.
We first explain as much of a model's decision as possible using linear combinations of annotated concepts. We then learn a low rank subspace of the network's feature space, that, along with the semantic attributes, can explain most of the model.  Our approach can be thought of as a \emph{recursive} decomposition, where separating out the semantic information from pre-labelled concepts leaves us with the remaining unexplained components of the network that can then be explained using different methods. 


\begin{comment}
Consider a blackbox scene classification model as in Fig.~\ref{fig:pull_fig}. This model takes as input an image, and outputs a scene prediction. We want to understand how this model arrives at its decision. Given a set of semantic attributes (such as \texttt{table}, \texttt{person} or \texttt{sky}), ELUDE (Explanation via a Labelled and Unlabelled Decomposition) decomposes model's prediction into a linear combination of these labelled attributes as well as some `un-interpretable` CNN features that do not contain any information about these attributes. This then allows us to examine the `un-interpretable` features in more depth to understand what other attributes the model might be using. 
\end{comment}


%\smallsec{Importance of interpretability} It is well-established that deep learning models achieve excellent performance across a wide range of tasks. However, they remain notoriously difficult to interpret and understand: they are over-confident in their mistakes~\cite{}, susceptible to surprising adversarial attacks~\cite{}, XXX. This lack of reliability limits their use in real-world applications which require high-stakes decisions such as healthcare or XX~\cite{}. Despite impressive results on existing benchmarks, interpretability remains a key roadblock in unlocking the full potential of deep learning. 

%\smallsec{Diversity of methods} Multiple methods have been proposed for interpreting and better understanding deep neural networks~\cite{selvaraju2017gradcam,bau2017netdissect,...}. %NetDissect explains individual neurons of a network through correlating their XXX, and is evaluated by YYY. Method AAA does BBB and is evaluated by ZZZ...
%These methods have taken a wide range of approaches including explaining individual neurons of a network~\cite{}, visualized pixels that contribute to particular decisions~\cite{}, XXX. They have been evaluated in different quantitative and qualitative ways, including human studies~\cite{}, correlations with pre-annotated image regions~\cite{}, human interventions, XXX.
%The proliferation of interpretability methods is heartening, with each one bringing unique strengths, insights and evaluation metrics.

%\smallsec{Dominant paradigm} One dominant factor that remains the same across all interpretability literature is the focus on quantifying and discovering what \emph{can} be explained about the model's decisions. 
%NetDissect explains N neurons of the network. ConceptBottleneck routes all decisions through M semantic attributes, allowing for interventions with X\% accuracy. 
%Every method explores and summarizes the discovered patterns that are correlated with the network's predictions, and notes that the network is not yet fully explained. However, was is frequently missing is the analysis of what \emph{cannot} be explained by each method. On one hand, explaining more and more of the network is the key goal of interpretability so it makes sense to focus on the positive explanations. On the other, as we argue in this work, there is a lot of overlooked value in quantifying and analyzing what patterns cannot yet be explained by the network. %Similar to works analyzing the \emph{errors} of object detection~\cite{Hoiem12,TIDE} 

%What other information is hiding in the network that is not being captured? %How much? %Are different methods explaining the same or different parts of the network? What would a roadmap to \emph{complete} interpretability look like?



%\smallsec{Key questions} Studying the interpretability literature  leaves us with two key questions:
%\begin{enumerate}
%    \item Can we understand what remains \emph{unexplained} by the different methods? For example, if N neurons are explained, what are the remaining X-N neurons doing? 
%    \item Can we quantify \emph{how much} is explained by the different methods, in a way that is compatible and comparable across the different models?
%\end{enumerate}


%




\begin{comment}
\smallsec{Our approach} %We present a meta-tool for studying interpretability methods. \olga{Similarly, adjust, it's not a meta-tool, it's a new method} 
We present a new global interpretability method that analyzes what parts of a network's prediction is and isn't explained by a set of pre-annotated semantic concepts. Given these concepts, 
%Given a set of pre-annotated semantic concepts, 
we first explain as much of the model's decision as possible using linear combinations of these concepts. This is similar to the approach in ConceptBottleneck~\cite{koh2020conceptbottleneck} with a few key differences due to our focus on understanding what remains \emph{unexplained} rather than enabling effective interventions. First, we are not interested in approximating the concepts (as that obscures some of the information) but in working directly with the accurate annotations. Second, we develop a method for ensuring that the remaining parts of the network do not contain any information about the semantic attributes. Given this decomposition, we apply visualization methods to understand what remains in the network. Our approach can be thought of as \emph{recursive} decomposition, where separating out the semantic information from pre-defined categories leaves us with the remaining unexplained components of the network that can then be explained using different methods. 

\smallsec{Summary of contributions} 
\end{comment}




%\smallsec{Key challenges} There are three key remaining challenges in interpretability which we set out to tackle in this work.
%\begin{enumerate}
%    \item \emph{Consistency.} The current methods are evaluated 
%\end{enumerate}

%They rely on pre-annotated semantic parts or attributes~\cite{XXX}, XXX... They focus on explaining as much of the network's decision as possible, and are evaluated with human studies~\cite{}, correlation with pre-annotated image subregions~\cite{}, XXX... Results are reported and compared across methods in terms of number of neurons that are explained or XXX. 

%One key aspect in the interptetability literature that is notoriously missing though is the quantification or understanding of the \emph{remaining,} yet-unexplained part of the network. For example,
%\begin{enumerate}
%    \item How much of the network's score has been explained and how much is attributed to the black-box remaining parts?
 %   \item Under what conditions is the network relying more on the interpretable parts of the model versus resorting to the black-box system? 
%\end{enumerate}


==> sections/method_old.tex <==

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/method_v8.png}
    \caption{An overview of our method (bottom right) compared to a baseline CNN, NetDissect~\cite{bau2017netdissect}, and Concept Bottleneck~\cite{koh2020conceptbottleneck}.} 
    \label{fig:methods}
\end{figure}

\iffalse
\begin{figure}[t!]
\centering
\begin{minipage}{.6\textwidth}
  \centering
  \includegraphics[width=\linewidth]{CompleteInterpretability/figs/method_v8.png}
\end{minipage}%
\begin{minipage}{.4\textwidth}
  \centering
  \includegraphics[width=\linewidth]{CompleteInterpretability/figs/rebuttal_graphic_take3.png}
\end{minipage}
\caption{\emph{(left)} An overview of our method (bottom right) compared to a baseline CNN, NetDissect~\cite{bau2017netdissect}, and Concept Bottleneck~\cite{koh2020conceptbottleneck}. \emph{(right)} We demonstrate how we learn $f'$ from $f$. As described in the main text, $X$ is a set of images, $A$ is a map from $X$ to $\{0, 1\}^K$ encoding $K$ semantic attributes, $f$ is the output of the penultimate feature layer of the blackbox model, $\epsilon$ is a hyperparameter we use to threshold the accuracy of any linear classifier.}
\label{fig:methods}
\end{figure}
\fi
%In this work, we introduce a new interpretability method that allows us to analyze what is and isn't explained by a set of semantic concepts.
%we set out to study what is \emph{not} explained by current interpretability approaches. \olga{Adjust: we introduce a new interpretability method that allows us to analyze what is and isn't explained by a set of semantic concepts.} 

\iffalse
* Goal 1: Explain a model's predictions using combination of semantic and continuous features
* Want to predict model's distribution, not just final output (Why?) 
* Explain how + why?
    * Learn linear regression for attributes
        * for simplicity add L1 penalty
    * Learn linear regression for remainder. 
        * For simplicity, add rank constraints. 
* Ideally, since attributes are forced to explain as much of the network as possible, this new low rank projection should not have any information about feature space. 
* Goal 2: Explaining multiple heads of a classifier with the same feature representation. 
    * Can this low rank subspace we compute be the same across all these heads? 
    * (Spoiler - yes)
    * Additive losses.
* Goal 3: Suppose we don't know all heads before hand: example transfer learning. Can we still find a reasonable subspace? 
    * Null projections? 
    * learn on all known, test out on unknown? 

\fi


%\smallsec{Overview} 
\subsection{Predicting a model's output}
Given a CNN image classification model $F$ and a set of semantic attributes, our goal is two-fold: first, we want to explain the scores of the network as much as possible using the provided attributes, and second, we want to learn a simple representation for the parts of the network that \emph{cannot} be explained by these attributes, so that they can then be visualized and examined in isolation. To do so, we will assume we have access to a set of images (typically not from the training set of $F$), for which we have  $K$ binary semantic attribute labels $A(x) \in \{0,1\}^K$ annotated in each image. {Like previous works~\cite{koh2020conceptbottleneck,fong2018net2vec,zhou2018ibd,kim2018tcav}, we also assume that the labelled attributes are encoded linearly within the feature space; thus, we provide an explanation that is a linear combination of these attributes. } %We propose generating this explanation through a novel method ELUDE: Explanation via a Labelled and Unlabelled DEcomposition as follows. 

%we can compute the output $F(x)$ as well as 

%To do so, we rely on describing two popular methods, NetDissect~\cite{bau2017netdissect} (a post-hoc analysis framework) and Concept Bottleneck~\cite{koh2020conceptbottleneck} (an interpretable-by-design system) which seemingly accomplish one or both of these tasks, and describe the key challenges that still remain. Then we present our framework which tackles these challenges.

\smallsec{Explaining using attributes} We begin by articulating how much the model relies on semantic attributes when making decisions. For example, NetDissect~\cite{bau2017netdissect} (Fig.~\ref{fig:methods} top right) examines the neurons in the network post-hoc and identifies those that appear to respond strongly to the presence of one of the semantic attributes. Doing so on the penultimate layer of the network (which is fed into the final classifier layer) allows one to then use the corresponding linear classifier weights to infer the degree to which the network relies on each of these now-interpretable neurons in making its prediction. However, a neuron that does not appear to be responding to any semantic attribute may still be encoding important information relevant to one or more of the attributes; thus, we may be underestimating the contribution of the different attributes to the network's prediction.  

%We introduce a simple alternative of explicitly training a model to evaluate the contributions of each attribute. Concretely
Instead, given the provided images, we can train a model $h$ directly on the semantic attribute labels $A(x)$ to approximate the network predictions $F(x)$. This allow us to both see how well the output distribution of the original network can be approximated with the semantic attributes and evaluate the contribution of each using the linear weights of $h$. We train this linear model with an $L1$ penalty on the coefficients in order to make the explanation generated as simple as possible. 

%Concretely, consider a set of images $x$ (typically not in the original training set of the classification network), corresponding K binary semantic attribute labels $A(x) \in \{0,1\}^K$, and the original predictions of the network $F(x)$.

However, this forces the model $h$ to rely \emph{exclusively} on the semantic attributes; i.e., it does not allow for the possibility that the network is using any additional information. In fact, a recently-proposed interpretable-by-design Concept Bottleneck~\cite{koh2020conceptbottleneck} framework (Fig.~\ref{fig:methods} bottom left) attempts to do this, by training a network where an intermediate layer has only $K$ neurons trained to correspond to the $K$ labelled semantic attributes. In practice, this leads to additional visual information being encoded in these neurons, making it significantly more difficult to properly interpret each one. To avoid this, we will need to provide the function $h$ with additional visual features $f'(x)$, described below, beyond the annotated attribute labels $A(x)$. 

%The second, arguably simpler concern is that the attribute labels $A(x)$ may be overcomplete; i.e., they may contain semantic attributes which are not in fact encoded or used by the network. Ideally, the function $h$ would then learn weights of $0$ for them; however, in practice $h$ is likely to leverage the spurious correlations and make use of them without providing any meaningful insight into the behavior of the network. To avoid this, we first consider $F(x) = g(f(x))$ where $g$ is the final linear classifier and $f(x)$ is the output of the penultimate feature layer, and train $K$ linear models on $f(x)$, corresponding to each semantic attribute $A_k(x)$. If a model cannot be trained above random chance for a given attribute $k$, we then know definitively that that attribute is not included in the learned decision space $F(x) = g(f(x))$ which we are aiming to interpret, and thus we discard the semantic attribute $k$ from $A$. 

\smallsec{Contribution of the remaining features}
We propose to learn $h$ as a sum of two linear models - one that relies exclusively on $A$, and another that relies exclusively on the uninterpretable features $f$, i.e, we maximize the objective 
\[\max_{W_A, W_f} Pr_x \big(F(x) = W_A^TA(x) + W_f^Tf(x)\big)\] This formulation of $h$, however, has an extremely simple solution - this could simply use the final linear layer of $F$ as $W_f$, ignoring $A$ altogether, which would not allow us to gain any information about the $F$. We thus train these in sequence, forcing $W^T_AA(x)$ to approximate $F(x)$ as well as possible first, before learning $W_f$. Another concern is that $W_f$ is as hard to explain as the original black box model. We address this concern by limiting the rank of $W_f$, by forcing it to be $W_f = U^TV$, with $U$ having rank $r$. Our final optimization therefore looks as follows:
\begin{align}
\label{eq:objection_single}
\max_{W_A} & \Big[Pr_x \big(F(x) = W_A^TA(x) \big) + \lambda_2 ||W_A||_1\Big] \\
    \max_{ U, V| rank(U)=r} &  Pr_x \big(F(x) = W_A^TA(x) + (U^TV)^Tf(x)\big)  
\end{align}
The low rank of $U$ implies the features within the model that do not correspond to the attributes in $A$ can be represented as $U^Tf$, thus giving us a simpler feature space that remains to be explained. The overall linear explanation of $h$ allows us to (1) quantify how much of $F(x)$'s decision can be attributed to the semantic attributes, (2) characterize the relative contribution of each attribute $A_k$ by the corresponding linear weight of $h$, and (3) visualize and analyze the learned space $U^f(x)$ to identify what additional information is being used in the network's decisions.  Together this creates a global explanation that allows humans to approximately predict model behavior given a new image. While certain interpretable-by-design models~\cite{chen2018protopnet,koh2020conceptbottleneck,nauta2021prototree} also allow this, our explanation is arguably simpler and more complete, as we explicitly separate out the semantic attributes and additional visual features. In addition, while  we stick to the labelled semantic attributes in this work, $A$ can potentially be replaced with other learned concepts such that the prototypes in Chen \etal~\cite{chen2018protopnet} or Nauta \etal~\cite{nauta2021prototree}, or the concepts identified by Ghorbani \etal~\cite{ghorbani2019ACE}. Most importantly, our approach allows us to explicitly study both the information which \emph{is} and \emph{is not} explained by the given attributes. 

\subsection{Beyond explaining single models}
\label{sec:beyond_single}
An advantage of our method is that the subspace $U^Tf$ contains information from $f$ not present in $A$. Thus, we can ask if a projection $U$ can be learned, such that $[U^f, A]$ can be used to explain multiple models that are trained with the same feature representation. One can imagine this setting arising when we use transfer learning to train models for small datasets. 

\smallsec{Known models}
We first tackle the scenario when we are given access to all these models when learning the subspace. Let $F^i = g^i o f$ for $i \in \{1, 2, \ldots m\}$. We want to produce a global explanation for each that uses the same uninterpretable subspace $U$ of $f$, along with the attributes $A$. In this case, we optimize Equations~\ref{eq:objection_single} over all the different $F_i$'s, keeping $U$ the same across these objectives:
\begin{align}
  \max_{W^i_A} & \Big[Pr_x \big(F^i(x) = (W^i_A)^TA(x) \big) + \lambda_2 ||W^i_A||_1\Big] & \forall i \in \{1, 2, \ldots m\} \\
    \max_{U, V^i|rank(U)=r} &  Pr_x \big(F^i(x) = (W^i_A)^TA(x) + (U^TV^i)^Tf(x)\big)   &  \forall i \in \{1, 2, \ldots m\}
\end{align}

\smallsec{Learning $U$ without $F$} 
However, in most cases, we might not have access to all of the models at training time. One option might be to use all the $F^i$'s we have access to during training to learn this subspace, hoping that the combination of these classifiers might encode enough information from $f$. Consider the case when we want to extract a subspace $U^Tf$ from a feature space $f$ that, along with the attributes $A$ can be used to explain any model trained on $f$, without access to $F$. Here, our goal is to extract $U^Tf$ such that it contains no information about the attributes $A(x)$ while containing as much additional visual information as possible. To do so, we adopt a greedy approach. Given an attribute $A_k$, we train a linear model on $f(x)$ to approximate $A_k(x)$. We then project $f(x)$ into the null space of the learned hyperplane. Ideally this space would contain no information about this attribute; however, works such as Zhu \etal~\cite{zhu2017prune} have shown that a feature space often contains redundant information, and there could be multiple linear hyperplanes that approximate each attribute. Thus, we repeat this step (learning the hyperplane and projecting it onto the null space of the coefficients), until the AUC of the learned classifier is worse than a threshold $t$. This gives us a set of directions in $f$ that can be approximated by $A_k$. We repeat this process for all attributes in $A$. After this process, we have a set of directions in $f$ which can be approximated by the attributes in $A$. 
We then compute the null space of all these directions, and use this projection as $U$. By construction, $U^f(x)$ does not linearly encode information about the semantic attributes $A(x)$. This new feature space $U^Tf$ can thus be combined with $A$ to explain any linear model trained on $f$. 


==> tables/CAM_ad.tex <==

\begin{tabular}{l p{1.6cm}p{1.6cm}p{1.6cm} p{10pt} p{1.6cm}p{1.6cm}p{1.6cm}}
& image & \begin{tabular}{c}
     orig \\ heatmap
\end{tabular} & \begin{tabular}{c}
     remaining \\ heatmap
\end{tabular} && image & \begin{tabular}{c}
     orig \\ heatmap
\end{tabular} & \begin{tabular}{c}
     remaining \\ heatmap
\end{tabular} \\
\begin{tabular}{l}
\texttt{shopping}\\ \texttt{dining} 
\end{tabular} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/0_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/0_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/0_0.png}} && %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/0_1.png}} & %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/0_1.png}} & %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/0_1.png}} && 
\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/0_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/0_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/0_2.png}} \\
\begin{tabular}{l}
\texttt{home}\\ \texttt{hotel} 
\end{tabular} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/2_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/2_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/2_0.png}} && %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/2_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/2_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/2_1.png}} && 
\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/2_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/2_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/2_2.png}} \\
\begin{tabular}{l}
\texttt{mountains}\\ \texttt{desert} \\\texttt{sky} 
\end{tabular} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/7_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/7_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/7_0.png}} && %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/7_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/7_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/7_1.png}} && 
\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/7_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/7_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/7_2.png}} \\
\begin{tabular}{l}
\texttt{forest}\\ \texttt{field} \\\texttt{jungle} 
\end{tabular}  & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/8_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/8_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/8_0.png}} && %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/8_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/8_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/8_1.png}} && 
\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/8_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/8_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/8_2.png}} \\
\begin{tabular}{l}
\texttt{cabins}\\\texttt{gardens} \\\texttt{farms} 
\end{tabular}  & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/14_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/14_0.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/14_0.png}} && %\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/14_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/14_1.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/14_1.png}} && 
\raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/images/14_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/orig/14_2.png}} & \raisebox{-.5\height}{\includegraphics[width=1.4cm]{figs/CAM_ade20k/remain/14_2.png}} \\
\end{tabular}
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_orig/img22.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_both/img22.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_orig/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_both/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_orig/img21.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_5_both/img21.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_orig/img19.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_both/img19.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_orig/img8.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_both/img8.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_orig/img5.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_6_both/img5.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_orig/img24.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_both/img24.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_orig/img5.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_both/img5.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_orig/img20.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_7_both/img20.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_orig/img9.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_both/img9.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_orig/img6.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_both/img6.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_orig/img12.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_8_both/img12.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_orig/img7.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_both/img7.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_orig/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_both/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_orig/img5.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_9_both/img5.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_orig/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_both/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_orig/img15.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_both/img15.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_orig/img3.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_10_both/img3.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_orig/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_both/img25.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_orig/img11.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_both/img11.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_orig/img24.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_11_both/img24.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_orig/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_both/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_orig/img12.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_both/img12.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_orig/img24.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_12_both/img24.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_orig/img14.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_both/img14.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_orig/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_both/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_orig/img17.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_13_both/img17.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_orig/img12.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_both/img12.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_orig/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_both/img27.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_orig/img19.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_14_both/img19.png} \\
%& \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_orig/img15.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_both/img15.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_orig/img3.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_both/img3.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_orig/img9.png} & \includegraphics[scale=0.2]{figs/CAM_ade20k/scene_15_both/img9.png} \\

==> tables/ade_imp_old.tex <==
\begin{tabular}{l c l}
    \toprule
    Scene group & TPR(\%) & Important attributes \\
    \toprule
    \texttt{home-hotel} & 90.2 &   \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{arm}}},  \textcolor{NavyBlue}{\textbf{\texttt{hand}}} \\ %\textcolor{red}{\textit{\texttt{wood}}},  \textcolor{red}{\textit{\texttt{sky}}} \\
\texttt{water-ice-snow} & 82.4 &   \textcolor{NavyBlue}{\textbf{\texttt{ceiling}}},  \textcolor{red}{\textit{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{paper}}} \\ %\textcolor{red}{\textit{\texttt{wood}}},  \textcolor{red}{\textit{\texttt{building}}} \\
\texttt{commercial-buildings-towns} & 82.1 &   \textcolor{NavyBlue}{\textbf{\texttt{wood}}},  \textcolor{NavyBlue}{\textbf{\texttt{sky}}},  \textcolor{red}{\textit{\texttt{black}}} \\ %\textcolor{red}{\textit{\texttt{building}}},  \texttt{cnn-feature} \\
\texttt{outdoor-manmade-elements} & 75.0 &   \textcolor{NavyBlue}{\textbf{\texttt{ceiling}}},  \textcolor{red}{\textit{\texttt{black}}},  \texttt{cnn-feature} \\%,  \texttt{cnn-feature},  \textcolor{red}{\textit{\texttt{orange-c}}} \\
\texttt{forest-field-jungle} & 72.6 &   \textcolor{red}{\textit{\texttt{black}}},  \textcolor{red}{\textit{\texttt{painted}}}, \texttt{cnn-feature} \\ %,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{cultural-historical} & 71.0 &   \textcolor{NavyBlue}{\textbf{\texttt{wood}}},  \texttt{cnn-feature},  \texttt{cnn-feature} \\%,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{mountains-desert-sky} & 69.0 &   \textcolor{NavyBlue}{\textbf{\texttt{ceiling}}},  \textcolor{red}{\textit{\texttt{black}}},  \textcolor{red}{\textit{\texttt{red}}} \\%, \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{outdoor-transportation} & 67.0 &   \textcolor{red}{\textit{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{wood}}},  \textcolor{NavyBlue}{\textbf{\texttt{sky}}} \\%,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{indoor-sports-leisure} & 65.6 &   \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \texttt{cnn-feature},  \textcolor{red}{\textit{\texttt{sky}}} \\%,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{indoor-transportation} & 64.1 &   \textcolor{NavyBlue}{\textbf{\texttt{tree}}},  \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{person}}} \\%,  \textcolor{NavyBlue}{\textbf{\texttt{building}}},  \textcolor{NavyBlue}{\textbf{\texttt{arm}}} \\
 \texttt{workplace} & 63.9 &   \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \textcolor{red}{\textit{\texttt{ceiling}}},  \texttt{cnn-feature} \\%,  \textcolor{red}{\textit{\texttt{wood}}},  \textcolor{red}{\textit{\texttt{arm}}}, \\
    \texttt{shopping-dining} & 63.6 &   \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{windowpane}}},  \textcolor{NavyBlue}{\textbf{\texttt{building}}}\\%,  \texttt{cnn-feature}, \texttt{cnn-feature} \\
    \texttt{cabins-gardens-farms} & 62.5 &   \textcolor{NavyBlue}{\textbf{\texttt{wood}}},  \texttt{cnn-feature},  \texttt{cnn-feature}\\%,  \texttt{cnn-feature},  \textcolor{NavyBlue}{\textbf{\texttt{floor}}} \\
\texttt{outdoor-sportsfields-parks} & 60.6 &   \texttt{cnn-feature},  \texttt{cnn-feature},  \textcolor{NavyBlue}{\textbf{\texttt{sky}}}\\%,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{industrial-construction} & 55.4 &   \textcolor{NavyBlue}{\textbf{\texttt{wood}}},  \textcolor{NavyBlue}{\textbf{\texttt{painted}}},  \texttt{cnn-feature} \\%,  \texttt{cnn-feature},  \texttt{cnn-feature} \\
\texttt{indoor-cultural} & 54.3 &   \textcolor{NavyBlue}{\textbf{\texttt{black}}},  \textcolor{NavyBlue}{\textbf{\texttt{wall}}},  \texttt{cnn-feature} \\%,  \textcolor{NavyBlue}{\textbf{\texttt{building}}},  \textcolor{NavyBlue}{\textbf{\texttt{windowpane}}} \\
    \toprule
    \end{tabular}

==> tables/tab-review.tex <==
\begin{table}[ht]
\tiny
\centering
\input{main_table2}
\caption{We summarize key ideas behind several types of interpretability research over the past decade and compare them to our method ELUDE. We allow for humans to predict the model's output while also computing a feature space that is yet to be explained.}
\label{tab:review}
\end{table}
